Localized spatiotemporal reaction-diffusion patterns on a line and a disk arising from a subcritical finite wavenumber Hopf instability

Spatiotemporal localized and extended structures associated with a subcritical finite wavenumber Hopf bifurcation are studied in the Purwins model (a three-variable FitzHugh-Nagumo version). Steady and time-dependent numerical continuation procedures are used to investigate snaking behavior of localized standing and traveling waves on the real line, and the results are corroborated using weakly nonlinear theory. The results shed light on the origin of so-called jumping oscillons and the organization of a nontypical homoclinic snaking structure of traveling pulses. The computations are extended to moderate size disks and used to identify wall-attached spots that travel along the disk boundary as well as wall-attached spots that oscillate in place and wall-attached jumping oscillons. The one-dimensional results are shown to be useful in interpreting the two-dimensional results. Domain-filling and mixed structures are also studied, demonstrating the variety of extended and localized states that emerge in two-space dimensions, ranging from periodic to disordered. The latter are potentially important for observations of waves in far-from-equilibrium media, such as those often observed in cell biology.

==> ghtikz.tex <==
\usetikzlibrary{arrows.meta}
\tikzset{%
  >={Latex[width=1mm,length=3mm]},
% Specifications for style of nodes:
base/.style = {rectangle, rounded corners, draw=black,
                minimum width=3mm, minimum height=1mm,
%               text width=30mm, 
align=left},%, font=\sffamily},  
le/.style = {rectangle, rounded corners, draw=black,  
      minimum width=3mm, minimum height=5mm, %text width=10mm,  
align=left},
mi/.style = {rectangle, rounded corners, draw=black, % minimum width=3cm, 
    minimum height=2mm, %text width=32mm,  
align=left}, 
sm/.style = {draw=black, rounded corners, align=left},
ri/.style = {draw=black, rounded corners}
}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> mytikz.tex <==
% \usetikzlibrary{arrows,positioning} 
% \tikzset{
%     %Define standard arrow tip
%     >=stealth',
%     %Define style for boxes
%     punkt/.style={
%            rectangle,
%            rounded corners,
%            draw=black, very thick,
%            text width=6.5em,
%            minimum height=2em,
%            text centered},
%     % Define arrow style
%     pil/.style={
%            ->,
%            thick,
%            shorten <=2pt,
%            shorten >=2pt,}
% }

% \usetikzlibrary{calc,trees,positioning,arrows,chains,shapes.geometric,%
%     decorations.pathreplacing,decorations.pathmorphing,shapes,%
%     matrix,shapes.symbols}

% \tikzset{
% >=stealth',
%   punktchain/.style={
%     rectangle, 
%     rounded corners, 
%     % fill=black!10,
%     draw=black, very thick,
%     text width=10em, 
%     minimum height=3em, 
%     text centered, 
%     on chain},
%   line/.style={draw, thick, <-},
%   element/.style={
%     tape,
%     top color=white,
%     bottom color=blue!50!black!60!,
%     minimum width=8em,
%     draw=blue!40!black!90, very thick,
%     text width=10em, 
%     minimum height=3.5em, 
%     text centered, 
%     on chain},
%   every join/.style={->, thick,shorten >=1pt},
%   decoration={brace},
%   tuborg/.style={decorate},
%   tubnode/.style={midway, right=2pt},
% }


% \tikzset{%
%         brace/.style = { decorate, decoration={brace, amplitude=5pt} },
%        mbrace/.style = { decorate, decoration={brace, amplitude=5pt, mirror} },
%         label/.style = { black, midway, scale=0.5, align=center },
%      toplabel/.style = { label, above=.5em, anchor=south },
%     leftlabel/.style = { label,rotate=-90,left=.5em,anchor=north },   
%   bottomlabel/.style = { label, below=.5em, anchor=north },
%         force/.style = { rotate=-90,scale=0.4 },
%         round/.style = { rounded corners=2mm },
%        legend/.style = { right,scale=0.4 },
%         nosep/.style = { inner sep=0pt },
%    generation/.style = { anchor=base }
% }
% \newcommand\particle[7][white]{%
%   \begin{tikzpicture}[x=1cm, y=1cm]
%     \path[fill=#1,blur shadow={shadow blur steps=5}] (0.1,0) -- (0.9,0)
%         arc (90:0:1mm) -- (1.0,-0.9) arc (0:-90:1mm) -- (0.1,-1.0)
%         arc (-90:-180:1mm) -- (0,-0.1) arc(180:90:1mm) -- cycle;
%     \ifstrempty{#7}{}{\path[fill=purple!50!white]
%         (0.6,0) --(0.7,0) -- (1.0,-0.3) -- (1.0,-0.4);}
%     \ifstrempty{#6}{}{\path[fill=green!50!black!50] (0.7,0) -- (0.9,0)
%         arc (90:0:1mm) -- (1.0,-0.3);}
%     \ifstrempty{#5}{}{\path[fill=orange!50!white] (1.0,-0.7) -- (1.0,-0.9)
%         arc (0:-90:1mm) -- (0.7,-1.0);}
%     \draw[\ifstrempty{#2}{dashed}{black}] (0.1,0) -- (0.9,0)
%         arc (90:0:1mm) -- (1.0,-0.9) arc (0:-90:1mm) -- (0.1,-1.0)
%         arc (-90:-180:1mm) -- (0,-0.1) arc(180:90:1mm) -- cycle;
%     \ifstrempty{#7}{}{\node at(0.825,-0.175) [rotate=-45,scale=0.2] {#7};}
%     \ifstrempty{#6}{}{\node at(0.9,-0.1)  [nosep,scale=0.17] {#6};}
%     \ifstrempty{#5}{}{\node at(0.9,-0.9)  [nosep,scale=0.2] {#5};}
%     \ifstrempty{#4}{}{\node at(0.1,-0.1)  [nosep,anchor=west,scale=0.25]{#4};}
%     \ifstrempty{#3}{}{\node at(0.1,-0.85) [nosep,anchor=west,scale=0.3] {#3};}
%     \ifstrempty{#2}{}{\node at(0.1,-0.5)  [nosep,anchor=west,scale=1.5] {#2};}
%   \end{tikzpicture}
% }
